Beyond Agile: Studying The Participatory Process in Software Development

We see that the collaborative and participatory nature of software development continues to evolve, shape and be shaped by communication channels that are used by developer communities of practice--both by traditional communication channels (e.g., telephone, in-person interactions), as well as social features that may be standalone or integrated with other development tools (e.g., email, chat, and forums). Within a community of practice, software is a combination of the externalized knowledge (e.g., code, documentation, history of activities) as well as the tacit knowledge that resides in the community members' heads (e.g., experience of when to use an API, or design constraints that are not written down). Communication channels and development tools support developers in forming and sharing both externalized and tacit knowledge in a highly collaborative manner. However, not much is known about the impact this participatory culture is having on software development practices nor on the knowledge-building processes. The research community has been studying the tools and communication channels used by developers in an effort to broaden our understanding. But, studying only the tools and channels can only provide a narrow perspective. We believe that software development has evolved beyond the agile process, into a Participatory Process--A knowledge building process which is characterized by the (1) knowledge activities and actions, (2) stakeholder roles, and (3) is enabled by socially enhanced tools and communication channels. Thus, it is important to gain an understanding of each one of the components, and the way these components interact and shape each other.

==> 3-social-dev.tex <==
%!TEX root = candidacy.tex

\section{What We Know So Far} % (fold)
\label{sec:what_we_know}

In the following we present what we know on the participatory process in software development and its components. We highlight our work so far, and briefly describe the main findings. For each part, we indicate whether the work has been published, awaiting review, or partially completed.

\subsection{Communication Media Shapes the Participatory Process\\ in Software Development} % (fold)
\label{ssub:fose2014}
\begin{description}
\item \textit{This work has been published in Proceedings of ICSE 2014, FOSE track}
\end{description}

%First we need to gain an understanding of the past, present, and future roles of social media in software engineering---we need a research \textit{roadmap} to guide us. To that end, we provided a review of research that examines the use of different media channels in software engineering from 1968 to 2014~\cite{Storey2014}. We also report preliminary results from a large survey with developers that actively use social media to understand how they communicate and collaborate, and to gain insights into the challenges they face.

%We believe that social media in software engineering is contributing to a paradigm shift in three significant ways:
% \begin{enumerate}[noitemsep]
%     \item The rise of the social programmer that actively participates in online development communities;
%     \item A rapid increase in the creation and diffusion of technologies and crowdsourced content; and
%     \item The formation of ecosystems around content, technology, media, and developers.
% \end{enumerate}

First, we use the three types of knowledge described by Wasko \textit{et al.}~\cite{Wasko2000} to categorize how media support the flow of knowledge in software engineering. We also add a fourth type of knowledge that has recently become relevant in software engineering: \textbf{knowledge about people and social networks}.

\begin{figure}[h]
    \begin{center}
        \includegraphics[width=1.0\textwidth]{figures/fig_channels_over_time.pdf}
        \caption{Media channels over time and how they support the transfer of developer knowledge. Note that some channels overlap multiple types of knowledge communication.}
        \label{fig:timeline}
    \end{center}
\end{figure}

\subsubsection{Communicating Knowledge Embedded in People's Heads}

In the early history of software development, the main communication channel was \textbf{face-to-face}, as most groups and teams at that time were co-located. Furthermore, reliance on other members was not that significant as most programs written in the 1960s and early 1970s tended to be small~\cite{Shaw1996}. Face-to-face interaction was essential to support learning and problem solving, to build common ground~\cite{Clark1991} and to support collaborative system design and development. 
Face-to-face is often espoused to be the best way to exchange tacit knowledge, i.e., knowledge that resides in programmers' heads. Face-to-face interactions are still a mainstay of communication in software projects---however, many projects today are developed by engineers that may have never met face-to-face and never will. In some cases, video chat tools such as \textbf{Skype} or \textbf{Google Hangouts} are used as a substitute.

Another important communication channel between developers is \textbf{email}: \textit{``The big difference between a phone call and an electronic mail message is that the phone call interrupts and the e-mail does not. The trick isn't in the technology; it is in the changing of habits.''}~\cite{DeMarco1987} This tension between synchronous and asynchronous communication channels---and even workflows---is garnering renewed attention now that remote work and open source development models are being experimented with at young software companies (cf. e.g., Holman~\cite{Holman2011} about workflows at GitHub). \textbf{Instant messaging} is also used by many developers to support one-on-one discussions and exchange knowledge. Many developers also make use of \textbf{text-based group chat systems} for communicating about development, such as IRC. Tools that are popular today include the Web-based archivable Campfire\footnote{\url{https://campfirenow.com}} or HipChat\footnote{\url{https://www.hipchat.com}}.

\subsubsection{Communicating Knowledge Embodied in Project Artifacts}

In his landmark book \emph{The Mythical Man Month}, Brooks~\cite[p. 74]{Brooks1975} discussed the role of a \textbf{project workbook} as a comprehensive way to communicate knowledge embodied in a project artifact. The project workbook was used to document system knowledge, track all project activities, including rationale for design decisions and change information across versions. The workbook was eventually replaced with more sophisticated tools, notably \textbf{IDEs},  \textbf{online hyperlinked documentation}, \textbf{project forges}, \textbf{version control systems}, \textbf{bug trackers} and \textbf{project management} tools. Over time, these different tools incorporated various communication media and social features to support collaborative and distributed interactions. \textbf{Wikis} have been used to support defect tracking, documentation~\cite{Leuf2001}, requirements tracking, test case management and for the creation of project portals~\cite{Louridas2006}. Wikis are also used frequently in global software development~\cite{Lanubile2010} and remain integrated in collaborative and social coding sites~\cite{Lanubile2013}. 

In the free and open source world, \textbf{SourceForge}\footnote{\url{http://sourceforge.net}} has been widely used since 1999, and offers support for hosting projects and version control. And later, \textbf{GitHub} has overtaken SourceForge as the largest code hosting site\footnote{\url{http://redmonk.com/sogrady/2011/06/02/blackduck-webinar}}. For projects and teams, GitHub fosters collaboration through several awareness features, integration with external tools and support for asynchronous workflows (cf. e.g., Pham et al.~\cite{Pham2013}). \textbf{Email lists} have played an ongoing role in keeping members up to date with project activities. They have been used as a channel to disseminate commit logs from software repositories~\cite{Gutwin2004}, supporting project awareness and coordination. They have also been used for asynchronous code review in open source projects by sending small patches to members for review~\cite{Rigby2011,Rigby2012}.

Gutwin \textit{et al.}~\cite{Gutwin2004} also noted that important information about code was sometimes fragmented across the three channels used in those projects (email lists, chat and commit logs). Their study found that it was often difficult to ensure that information was read by the right people in a timely fashion. We suspect that fragmented communication may be an even bigger concern today given the increase in the number of communication channels used by many developers.

\subsubsection{Communicating Knowledge Socially Constructed in Community Resources}

\textbf{Usenet} was developed in 1980 as a ``worldwide distributed Internet discussion system'' and soon supported the flow of knowledge about technologies and projects across team, project, and community members. Users could read and post threaded messages, and posts were referred to as ``news'' belonging to specific categories or ``newsgroups''. It was a precursor to \textbf{forums} that are more widely used in recent years. Usenet differed from other \textbf{bulletin boards} at the time as it did not rely on a central server and a dedicated administrator: it was distributed among a network of servers that stored and forwarded messages to one another using ``news feeds''. But in other ways, it resembled the asynchronous text-based discussions on bulletin boards. 

Wasko et al.~\cite{Wasko2000}, in 2000, studied how Usenet played a role in knowledge management in three development communities of practice. In their survey, they found various reasons for participation: tangible returns such as the speed in getting multiple answers to questions, staying up to date, interaction with the community, reciprocity, 
%---not necessarily from a person they helped, but possibly someone else---, 
%being pro-social and helping the community, 
enjoyment, as well as enhanced reputation. 
% to gain different perspectives on a technical issue, and to keep up to date. 

%Some barriers were also noted: social clashes, but also technical barriers. 
Web-based archiving of Usenet posts began in 1995 at Deja News, which was acquired in 2001 by Google; the archives are now accessible by Google Groups. However, \textbf{Google Groups} is more than a gateway to Usenet archives---it provides discussion groups, mainly used as forums and mailing lists for software developers, and serves as a collaboration tool for global software engineering~\cite{Lanubile2010}. 

Many of the features in Usenet can now be seen in more modern media---most notably, \textbf{Stack Overflow}, a question and answer Website. Stack Overflow was created in 2008 and has experienced rapid uptake. Even though Stack Overflow has many parallels to Usenet, it differs in several important ways. Firstly, there is moderation of both questions and answers, which improves the trustworthiness and value of the content. Secondly, Stack Overflow has a gamification~\cite{Deterding2011} aspect with reputation scores and the ability to earn new powers through participation, which may encourage involvement through intrinsic and extrinsic motivation. Finally, the Stack Overflow community responds very quickly: over 92\% of questions are answered within a median time of 11 minutes~\cite{Mamykina2011}. Recently, Stack Overflow has been studied by several researchers~\cite{Mamykina2011,Barzilay2011,Cleary2013,Zagalsky2012} and is rapidly growing into a formidable documentation resource. E.g., Parnin et al.~\cite{Parnin201X} find that it provides very good coverage for documentation on open source APIs. 

Stack Overflow and many of the other channels mentioned in this section use a feature that was somewhat of a poster child for Web 2.0: \textbf{Folksonomies}~\cite{Peters2009}, also known as collaborative tagging or social bookmarking, comprise a user-generated system of classifying and organizing online content into different categories by using metadata such as tags. 
%Mathes~\cite{Mathes2004} explains that folksonomies are simply the set of terms that a group of users tagged content with; they are not a predetermined set of tags or labels, there is no hierarchy, and no directly specified parent-child or sibling relationships between them. There are, however, automatically generated ``related'' tags which cluster tags based on similar or related usage. 
What began with Delicious and Flickr in 2003 and 2004, respectively, soon spread to many other tools and Websites. In previous work, we studied the potential for \textbf{social tagging} in the IDE~\cite{Storey2006} and the use of tags for work item management in Jazz~\cite{Treude2009}. 

%\todo[inline]{Research on shared waypoints and social tagging to support collaboration \cite{Storey2006,Storey2006B}…}

%\todo[inline]{Folksonomies … many of the channels we mentioned used a feature that was somehwat of a posterchild for web 2.0 … folksonomies / collaborative tagging in delicious [2003; social bookmarking] and flickr [2004; photo sharing], then everywhere else. stack overflow, IDEs, … e.g. see [Treude2009], [Treude2012] for work item tagging in IDEs, maybe [Mamykina2011] has something on tags in SO?  TagSEA, Tours paper, and Tag Recommendation in Software Information Sites}

\textbf{Blogs} are another important community-based knowledge resource used in software engineering. First used in 1994 and widely adopted by 1999, with blogs, everyone can broadcast. They are frequently used by developers to document ``how-to'' information, to discuss the release of new features and to support requirements engineering~\cite{Park2009}. Moreover, some practitioners advocate that every developer should have a blog\footnote{\url{http://bit.ly/Every-Developer-Needs-a-Blog}}, arguing that blog posts help exchange technical knowledge among a larger audience than email messages. 
Pagano and Maalej~\cite{Pagano2011} examined both blogs and commit messages and found a relationship between blogging and commit behavior. 
%42\% of blog posts discussed functional requirements and domain concepts, 38\% discussed community news, and 30\% discussed APIs and project documentation. Source code was seldom discussed, higher level concepts were more prevalent. 15\% of blogs contain information already discussed in commit messages, and dependencies between the two decrease over time. 
Parnin and Treude~\cite{Parnin2011} found that blogs play an effective role in documenting APIs.
%: by analyzing the Google results for API calls of the jQuery API, they found that 87.9\% of the API methods were covered by blogs, mainly featuring tutorials and personal experiences about those API methods. 

Audio and video \textbf{podcasts} are a medium closely related to blogs and 
%, initially intended as digital audio broadcasts for portable music players like the iPod. However they are not limited to audio files alone, but can be used to distribute image or video files as well. 
used by software developers in a similar fashion: for learning~\cite{Lakhal2007}, keeping up to date with the latest trends and technologies~\cite{Wilson2008}, for (job) training and as how-to guides. Podcast use in higher education has increased since 2005~\cite{Campbell2005,Bongey2006}.
% and has been shown to be effective~\cite{Lakhal2007}.

\textbf{Social news Websites} are another medium experiencing a recent surge in popularity. Many of these sites~\cite{Virasoro2011} and aggregators allow developers to disseminate knowledge, discover new software and keep up to date. Some of the most popular among developers are Digg\footnote{\url{http://digg.com}}, reddit\footnote{\url{http://www.reddit.com}}, and Hacker News\footnote{\url{https://news.ycombinator.com}}. 
Lampe and Resnick~\cite{Lampe2004} analyzed Slashdot\footnote{\url{http://slashdot.org}}, a precursor to modern news Websites, and found that the basic concept of distributed moderation works well. However, their analysis revealed that it often takes a long time to identify especially good comments, that incorrect moderation activities are often not reversed, and that non top-level comments and comments with low starting scores did not receive as much consideration from moderators as other comments did. 

%Lerman~\cite{Lerman2007} examined the incentives that drive user participation on Digg and found competition with other community members, social acceptance, and internal factors. Findings also indicated that user participation is non-uniformly distributed with a few top users doing a large fraction of the work. Gilbert~\cite{Gilbert2013} studied Reddit votes and found a widespread underprovision of votes on Reddit, where half of the most popular links were overlooked the first time they were submitted, thus jeopardizing its main purpose. 
The importance of news Websites like Hacker News for software projects is beyond aggregating news and keeping up to date, as reaching the top of a site can provide valuable feedback and help the growth of a project's users, contributors and the community as a whole. These sites are a specific form of \emph{social navigation}, which was first defined by Dourish and Chalmers~\cite{Dourish1994} as movement from one item to another when provoked as an artifact of the activity of another or a group of others. 
%Dieberger et al.~\cite{Dieberger2000} discuss social navigation as a design approach to building software systems. 

%\todo[inline]{[ note there doesn't seem to be a paper on hacker news OPPORTUNITY! ]}

\textbf{Microblogging} is another channel that plays an increasingly important role in curating community knowledge. Twitter, the first microblogging tool and one of the most popular social media channels, was created in 2006 as a way to share short messages with people in a small group. The idea was to share inconsequential ephemeral information, but it has become an important medium in many domains. Twitter is seeing significant adoption in software engineering. 

Several researchers have investigated how software developers and software projects make use of Twitter~\cite{Bougie2011,Wang2013}, finding that Twitter is used to communicate issues, documentation, to advertise blog posts to its community, as well as to solicit contributions from users.
% Bougie et al. found that developers use it in quite different ways from the average population~\cite{Bougie2011}. 
%Wang et al.~\cite{Wang2013} analyzed tweets associated with the Drupal open source content management system and found that the Drupal project uses Twitter to communicate issues, documentation, and blog posts to its community, as well as to solicit contributions from users. 
In a recent study~\cite{Singer2013a}, we 
%reported on the perceived benefits that Twitter brings to adopters of Twitter for software engineering, as well as insights on why others reject it. We 
found that developers who adopted Twitter use it to filter and curate the vast amount of technical information available to them. We found it brought benefits in terms of awareness, learning, and relationship building. 
Developers who feel that Twitter benefits them rely on a variety of strategies for posting and reading Twitter content. 
%
Twitter shares some commonalities with Usenet, in that people join Twitter to discover information, to stay up to date and to be part of the community. Yet, Twitter is also quite different from newsgroups. With Twitter, users follow individuals, but create the community they wish to be a part of themselves. Twitter also includes a few signals that can help assess content and people, such as a user's number of followers or the number of retweets for an individual tweet. 
%Twitter supports only lightweight conversations; our research on Twitter~\cite{Singer2013a} revealed that developers switch to other channels for longer conversations. 

Social media is not only a disruptive force for developers, but also for enterprises. However, applying social media concepts in enterprise environments raises various concerns (e.g., privacy, security, distractions, ownership, etc...), which has led to the emergence of Enterprise Social Media~\cite{Leonardi2013}. These are social media adjusted for use in enterprise contexts that try to mitigate some of the concerns. 
\textbf{Yammer}\footnote{\url{https://www.yammer.com}} is a microblogging service much like Twitter, but designed for corporate use. Zhang et al.~\cite{Zhang2010} investigated how employees of a large enterprise use Yammer and how its usage differs from Twitter. They found that employees use Yammer for news about groups and less for posting content about themselves. 
%Conversations on Yammer seem to be longer than on Twitter. Study participants reported that Yammer helps them stay aware of what colleagues are  working on, and that it helps them make new connections. 
% could skip the mood based one…
%Other microblogging tools are used in software engineering, such as as the one described by 
Dullemond et al.~\cite{Dullemond2013} also studied the use of a microblogging tool within a small distributed software company where moods are communicated explicitly as part of posts. 

%\todo[inline]{[possible remove this as this is not from a paper or journal] Gartner Inc., an information technology research and advisory company, predicted in 2010 that by 2012, over 50 percent of enterprises will use activity streams that include microblogging, but stand-alone enterprise microblogging will have less than 5 percent penetration [ref].

%[more references for enterprise social software: Enterprise Social Media: Definition, History, and Prospects for the Study of Social Technologies in Organizations, Knowledge Sharing and Collaboration among Employees Using Enterprise Social Software (G Harden - 2013), The Role of Enterprise Social Media in the Development of Aerospace Industry Best Practices, Modeling Microblogging Adoption in the Enterprise, A case study of micro-blogging in the enterprise: use, value, and related issues, Enterprise Social Networking: Opportunities, Adoption, and Risk Mitigation]

%Could talk about http://en.wikipedia.org/wiki/Enterprise\_social\_software enterprise social software as a different category?}

%Summary paragraph here to segueway to next section… we've now talked about knowledge in people, in projects, and in communities. now media that help communicating knowledge ABOUT people and their relationships. 

\subsubsection{Communicating Knowledge About Developers Through Social Networks}

Sites that are primarily focused around social networking features are becoming very popular in development communities---just as Facebook has been very popular with the general population. This kind of media is new in software engineering, although implicit social networks have been present in other media channels, such as through newsgroup or mailing list affiliations. However, with these new media, the affiliation is one of the primary features of the medium, and as such, is made visible. 
\textbf{Facebook} is used by some developers to support programming interactions, such as local meet-ups. Sites such as \textbf{LinkedIn} are more focused on professional connections, but Barzilay et al.~\cite{Barzilay2011} explored the practice of example usage in software development by observing software developers' exchanges in LinkedIn discussion groups. 

There are also specific sites designed to showcase developer activities and skills, such as \textbf{Masterbranch}\footnote{\url{https://masterbranch.com}} and \textbf{Coderwall}\footnote{\url{https://coderwall.com}}, while many other developer tools now also integrate social networking features, such as \textbf{GitHub}. 
Below, we summarize some recent studies that have studied the impact of social networking on software engineering.   
 
Dabbish et al.~\cite{Dabbish2012} conducted a study of GitHub users. They found that the visibility of developer activities and profiles on GitHub influences a project's success by motivating others to contribute. 
% evelopers to assess other developers and projects.  
Developers further decide which projects are worth contributing to by determining which projects have frequent contributions or  contributions from high status developers~\cite{Tsay2013}. High status developers are those that have already done interesting work. 
% Interviewees in this study said that a project's developers' visibility is important for the project to succeed. However, they did not value explicit self-promotion. Developers use others' profiles to assess their technical goals and vision. This allows them, for example, to better assess which of a few similar projects is more likely to be successful in the long term. Interviewees were also aware that others were watching their own projects in the same manner, which they said motivated them and made them conscious about the quality of their own code. 

%Tsay et al.~\cite{Tsay2013} analyzed the interviews from the aforementioned study with a focus on social signaling theory. They found that developers are interested in what projects high status developers contribute to, as their attention would ``mean something'' about a project's merit. High status developers had already proven that they do interesting work, so any project they worked on would likely be interesting as well. High status was inferred from a high follower count on GitHub and contributions to high profile projects. These interpretations would influence developers' propensity to contribute to one project instead of another. Similarly, projects are more attractive when they have developers that seem more committed than those of other projects. Developers inferred commitment for example from the frequency of a project's developers' contributions. Relatedly, the most active people were assumed to be the most important developers in a project and would therefore warrant more attention. 

In a similar study, Marlow et al.~\cite{Marlow2013a} explored how users on GitHub form impressions of others through GitHub's transparency. They found that developers assess each other to learn about projects and their status. These impressions guide future developer interactions and 
%and would help understanding what value a contact could have to oneself in the future. Interviewees said they used a developer's past activity across different projects to form these impressions and similarly to other studies said that contributions to high status projects made a developer seem more important. Such impressions would also 
influence how much one would trust contributions from someone they had not interacted with before. Pham et al.~\cite{Pham2013} interviewed GitHub users with regard to testing practices and found that when assessing contributions from others, project owners behave differently based on how much they trust the contributor. Unknown developers' code would be more thoroughly scrutinized than code from trusted people. 

Marlow and Dabbish~\cite{Marlow2013} studied how employers assess developers based on their GitHub profiles, which provide cues about their activities, skills, motivations and values. These cues were regarded as more reliable than resumes. 
% as activity is transparent on GitHub and manipulation of that activity is very costly and thus unlikely. 
Employers who were interviewed by Marlow et al. said that open source contributions indicated that a developer had the ``right'' set of values and was not in software development for purely financial reasons. 
%Activity in open source was interpreted as developers liking what they do and wanting to give back to the community. Again, 
Also, contributions to high status projects were said to demonstrate ``some level of proficiency.''
%, as that basically meant that a high status developer would vouch for someone's work. 
%However, interviewees were aware that on its own, a contribution is not a reliable indicator---one would need to look at the actual code to assess the real value of such a contribution. Study participants also realized that a project's success may also depend a lot on marketing efforts in social media from the project owners.

Singer et al.~\cite{Singer2013} conducted a similar study, but investigated social media profiles of developers in general. This included GitHub, 
%but also Twitter and developer 
profile aggregators such as Coderwall and Masterbranch, 
%sites that create an aggregated overview from activities on GitHub, 
Twitter, Stack Overflow, and other sites. 
They found that profiles can be hard to understand or evaluate for some recruiters. 
%Others were unsure still of their benefits, and some thought the sites would just provide an entry point. 
To assess the real merit of a developer's public activities, one would always need to look at actual artifacts, such as code, tests, documentation or discussions.
% to determine their passion for the work as well as their ability to learn quickly. 
%Recruiters said that when they assess developers, they want to find individuals who not only have the required technical skills, but who are also passionate, learn quickly, and have a diverse skill set---with the latter being a proxy for passion and quick learning. Developers also assessed other developers and were aware of that. 
Developers also assessed recruiters and companies, trying to gauge their authenticity and suitability as colleagues. Most developers and recruiters were aware that the absence of signals does not mean much---a developer with few or no public activities might just be a private person or work exclusively on closed source projects. 
%In our in-depth study concentrating on how developers use Twitter \cite{Singer2013a}, we again found the assessment aspect mentioned in the previous study. Proficient Twitter users use a developer's follower count, following count, and the ratio of those numbers as an indicator for how important that person is. Developers seek out high status developers on Twitter to learn from them in a casual manner and to stay current with technology. Finally, developers use Twitter to connect with others casually and also for finding job opportunities. 
%
Capiluppi et al.~\cite{Capiluppi2013} further argue that information that helps assess others will allow for more merit-based and less credential-based evaluation of potential candidates, possibly leveling the playing field for those who don't have access to traditional education but are skilled and desirable developers. 

Together with Begel and Bosch, we interviewed representatives of GitHub, the \textbf{Microsoft Developer Network (MSDN)}, \textbf{Stack Exchange} and \textbf{TopCoder} about the role of social networking in their companies~\cite{Begel2013}.
All four sites provide features to increase the visibility of developers and developer activities. On GitHub, one can follow particularly high status developers and watch their activities.  MSDN and Stack Exchange have explicit gamification elements to assist in assessment and discovery of content, and to support strong engagement. 
Interestingly, not having explicit connections between users was a conscious decision for Stack Exchange: the company feels users should concentrate on the content, and status should not play into a question or answer being up-voted.
The Stack Exchange interviewee mentioned that the hardest part about building the Stack Exchange Network was not creating the software that runs it---the challenge was building the community, its mechanisms, and the processes that support it. 
Similarly, the TopCoder\footnote{\url{http://www.topcoder.com}} representative also mentioned that building a functioning community was the most difficult aspect in building the business.   Both GitHub and Stack Overflow (the most notable of the Q\&A sites Stack Exchange hosts) relied on high status developers to seed their communities.

% On GitHub, one can see what projects others,   Other features in GitHub, such as the repository URL containing the creator's name and the use of avatars, helps build reputation and thus trust by others. 
% MSDN uses social networking features to connect developers using Microsoft's products with Microsoft's employees. The site also uses some gamification elements in the form of achievements and points---this gives users feedback about the value they have provided to the community. 
% The Stack Exchange Network runs a host of Q\&A sites, the most notable among them being Stack Overflow. Contrary to MSDN, gamification elements in Stack Overflow are not merely used for assessment and discovery of content, but for the creation of strong engagement: contributing high quality content earns a user reputation points, which in turn unlock new features on the site.  Through this mechanism, only involved users can access the more regulating functions, such as deleting or downvoting posts. This has a significant effect on user engagement, as it creates a sense of involvement and ownership among members. 

In summary, the pervasive use of public social media by developers makes the participants and their relationships more transparent to software engineering researchers who want to understand how methods and tools are used in practice. 
While the mining of software repositories has given us access to software products for a relatively long time, the recent accessibility of developers' interactions and their relationships can provide more qualitative insights than had previously been available.  Research so far has indicated that social networking features influence which projects developers participate in, impact project success, and play a role in developer assessment and recruitment.  Gamification elements add feedback and improve trust in developer contributions.  We believe studies on social networking and their associated gamification aspects will become more prevalent in the future of software engineering research, adding to these preliminary insights. 

\subsubsection{Methodology}

\subsubsection{Findings}

\subsubsection{Contribution}

help us understand the kinds of media channels this population uses to communicate and collaborate.

We consider the impacts of social media on software engineering activities.

This paper showcases a research roadmap that outlines opportunities and challenges arising from the use of social media in software engineering. We include a history of media use in software engineering, from the very first days of software engineering in the late 1960s, to the present day use of social media, preceded by a conceptual background on the role of media in communities. The paper concludes with a discussion on the impact social media is having on software engineering research directions and methods.

% subsection fose2014 (end)

\subsection{How Communication Channels Shape and Challenge A Participatory Culture in Software Engineering} % (fold)
\label{sub:dev_challenges}

% subsection dev_challenges (end)

\subsection{Why Developers Are Slacking Off: Understanding How Software Teams Use Slack} % (fold)
\label{sub:cscw2016_poster}

% subsection cscw2016_poster (end)

\subsection{The Rise of The Social Bots in Software Development} % (fold)
\label{sub:bots}

% subsection bots (end)

% section social_dev (end)

==> 4-social-research-education.tex <==
%!TEX root = candidacy.tex

\section{The Role of Social Media in Software Engineering Research and Education} % (fold)
\label{sec:social_research_education}

\subsection{Selecting Research Methods for Studying a Participatory Culture in Software Development} % (fold)
\label{sub:ease2015}

% subsection ease2015 (end)

\subsection{The Researcher's Guide: Conducting Empirical Studies in Software Engineering} % (fold)
\label{sub:meta_paper}

% subsection meta_paper (end)

\subsection{Qualitative Data Analysis Methods in Software Engineering} % (fold)
\label{sub:bellairs}

% subsection bellairs (end)

\subsection{The Emergence of GitHub as a Collaborative Platform for Education} % (fold)
\label{sub:cscw2015}

% subsection cscw2015 (end)

\subsection{Student Experiences Using GitHub in Software Engineering Courses: A Case Study} % (fold)
\label{sub:icse2016_seet}

% subsection icse2016_seet (end)

% section social_research_education (end)

==> 5-collaboration.tex <==
%!TEX root = candidacy.tex

\section{A Theory of Collaboration in Software Development} % (fold)
\label{sec:collaboration}

\subsection{Regulation as an Enabler for Collaborative Software Development} % (fold)
\label{sub:chase2015}

% subsection chase2015 (end)

\subsection{Using The Model of Regulation to Understand User-Developer Collaboration in a Software Project} % (fold)
\label{sub:icse2016}

% subsection icse2016 (end)

\subsection{Selecting Research Methods for Studying a Participatory Culture in Software Development} % (fold)
\label{sub:ease2015}

% subsection ease2015 (end)

\subsection{The Researcher's Guide: Conducting Empirical Studies in Software Engineering} % (fold)
\label{sub:meta_paper}

% subsection meta_paper (end)

\subsection{Qualitative Data Analysis Methods in Software Engineering} % (fold)
\label{sub:bellairs}

% subsection bellairs (end)

\subsection{The Emergence of GitHub as a Collaborative Platform for Education} % (fold)
\label{sub:cscw2015}

% subsection cscw2015 (end)

\subsection{Student Experiences Using GitHub in Software Engineering Courses: A Case Study} % (fold)
\label{sub:icse2016_seet}

% subsection icse2016_seet (end)


% section collaboration (end)
